Improving Arithmetic Reasoning Ability of Large Language Models through Relation Tuples, Verification and Dynamic Feedback

Current representations used in reasoning steps of large language models can mostly be categorized into two main types: (1) natural language, which is difficult to verify; and (2) non-natural language, usually programming code, which is difficult for people who are unfamiliar with coding to read. In this paper, we propose to use a semi-structured form to represent reasoning steps of large language models. Specifically, we use relation tuples, which are not only human-readable but also machine-friendly and easier to verify than natural language. We implement a framework that includes three main components: (1) introducing relation tuples into the reasoning steps of large language models; (2) implementing an automatic verification process of reasoning steps with a local code interpreter based on relation tuples; and (3) integrating a simple and effective dynamic feedback mechanism, which we found helpful for self-improvement of large language models. The experimental results on various arithmetic datasets demonstrate the effectiveness of our method in improving the arithmetic reasoning ability of large language models. The source code is available at https://github.com/gpgg/art.

==> latex/tables/gpt4o.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{ccc}
\hline
Backbone               & Method         & GSM8K         \\ \hline
\multirow{2}{*}{GPT4o} & ModelSelection & 96.2          \\
                       & Ours           & \textbf{96.6} \\ \hline
\multirow{2}{*}{Llama-3-8B-Instruct} & CoT & 80.1          \\
                       & Ours           & \textbf{80.4} \\                        
                       
                       \hline
\end{tabular}%
}
\caption{Accuracy results on GSM8K with different backbone models.}
\label{tab:gpt4o}
\end{table}
